Static and dynamic properties of 0, pi, and 0-pi ferromagnetic tunnel Josephson Junctions

We present experimental studies of static and dynamic properties of 0, pi and 0-pi superconductor-insulator-ferromagnet-superconductor (SIFS) Josephson junctions of small and intermediate length. In the underdamped limit these junctions exhibit a rich dynamical behavior such as resonant steps on the current-voltage characteristics. Varying the experimental conditions, zero field steps, Fiske steps and Shapiro steps are observed with a high resolution. A strong signature of the 0-pi Josephson junction is demonstrated by measuring the critical current as a function of two components (B_x, B_y) of an in-plane magnetic field. The experimental observation of a half-integer zero field step in 0-pi SIFS junctions is presented.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v2.00 -- LaTeX macros for frequently used
%%% abbraviations
%%%

\RequirePackage{xspace}

%stupid macros kike \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}


%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}
%big \frac called \ratio
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace} 
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}

%just shortcuts
\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

%Misc. macros to discuss with co-authors
\RequirePackage{changebar}
\newcommand{\X}[1]{}
%\newcommand{\Q}[1]{\cbstart {\small\sffamily Q: #1}\cbend}

%Misc. macros to discuss with co-authors
\newcommand{\Q}[1]{\par\noindent{\small\sffamily Q: #1}\par}
%\newcommand{\Q}[1]{}
\newcommand{\A}[1]{\par{\small\sffamily A: #1}\par}

%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}



